From Monolingual to Multilingual: Evaluating Mamba for ASR in South African Languages

Recent advances in automatic speech recognition (ASR) have explored different sequence models, including Conformer-based models and newer state space models such as Mamba. Although prior work has evaluated these architectures in multiple languages, their effectiveness in African languages remains underexplored. In this work, we evaluate Mamba for ASR on seven South African languages. In monolingual experiments, each model is trained on 50 hours of speech per language, and we compare Mamba to a Conformer baseline of similar parameter scale. Mamba achieves similar recognition accuracy to Conformer while using fewer computational resources and training faster. We further evaluate generalization in this setting and find that both models struggle to generalize to speech that is much longer than what they were trained on. We then study multilingual ASR using Mamba models, where the baseline is pooling all languages together. On top of this, we tested three extensions: training with language-family information by adding both language and language-family embeddings as biases to the downsampled acoustic representations, and multitask learning with a CTC ASR objective and a language identification (LID) head. We find that multilingual training consistently improves performance over monolingual training. However, adding explicit language information does not improve in-domain performance but does improve cross-corpus robustness. We conducted ablation studies in low-resource multilingual settings using 5-hour and 10-hour per-language training data, where we observed gains from using language embeddings and further demonstrated that removing or altering them hurt model performance. Lastly, we analysed these embeddings and find that they do not capture linguistic similarity in a typological sense, but instead act as task-specific control vectors.

==> eq.tex <==
\subsection{ASR Training Strategies}
Our experiments include both \textbf{monolingual} and \textbf{multilingual} training. For monolingual training, we trained a model on the sampled data for each language and evaluated it on the same language. Multilingual training includes four approaches:

\begin{enumerate}
    \item \textbf{Implicit} - combines all language data without any additional information.
    \item \textbf{Language tag} - Prepends a language-specific tag to each transcription during training in the form \texttt{$<$|language\_code|$>$}.
    \item \textbf{Hierarchical tag} - Prepends both the language family and the language tag to each transcription. For example, \texttt{$<$|nguni|$>$} for isiZulu, isiXhosa, and isiNdebele; \texttt{$<$|sotho|$>$} for Sesotho and Setswana; and \texttt{$<$|tsonga|$>$} and\texttt{$<$|venda|$>$} for Xitsonga and Venda.

% Investigation of Speaker-adaptation methods in Transformer based ASR
% Multilingual models with language embeddings for low-resource speech recognition
% Transformer ASR with Contextual Block Processing

    \item \textbf{Multitask learning} – the model is trained to predict both the transcription and language-related auxiliary targets simultaneously. The multitask loss is defined as:
    \begin{equation}
    \mathcal{L}_{\text{MTL}} = \mathcal{L}_{\text{CTC}} + \lambda \, \mathcal{L}_{\text{LID}}
    \end{equation}
    where $\lambda$ is a weighting factor (0.05, 0.1, or 0.2); we chose 0.1 as it performed best.
    
    A challenge in this setup is the difference in scale between the two losses, since $\mathcal{L}_{\text{CTC}}$ is generally much larger. To address this, instead of specifying $\lambda$ manually, we compute it dynamically based on the current loss ratio and a scaling factor $\alpha$:
    \begin{equation}
    \lambda = \mathcal{L}_{\text{CTC}} / \mathcal{L}_{\text{LID}} * \alpha
    \end{equation}
    where $\alpha$ is a small factor, typically set to 0.05, 0.1, or 0.2, to control the contribution of the auxiliary loss. Our ablation showed that this is not better than using a fixed $\lambda=1$.
